Karhunen-Loeve Analysis for Weak Gravitational Lensing

In the past decade, weak gravitational lensing has become an important tool in the study of the universe at the largest scale, giving insights into the distribution of dark matter, the expansion of the universe, and the nature of dark energy. This thesis research explores several applications of Karhunen-Loeve (KL) analysis to speed and improve the comparison of weak lensing shear catalogs to theory in order to constrain cosmological parameters in current and future lensing surveys. After providing a brief introduction to cosmology and to KL analysis, this work addresses three related aspects of weak lensing analysis: (1) Three-dimensional tomographic mapping (based on work published in Vanderplas et al. 2011); (2) Shear peak statistics with incomplete/gappy data (based on work published in Vanderplas et al. 2012); and (3) two-point parameter estimation from gappy data using KL modes (previously unpublished)... [this abstract has been abbreviated; please see the thesis for the full abstract].

==> dump.tex <==

\subsection{Fourier Transforms}
The Fourier Transform is a means of expressing a function in terms
of a certain class of oscillatory basis functions.
Given an arbitrary continuous function
$f(t)$, it can be re-expressed in terms of complex oscillatory basis functions
$\Phi_k(t) \equiv \exp[2\pi ikt]$
\begin{equation}
  \label{eq:FT_1D}
  f(t) = \int_{-\infty}^\infty \hat{f}_k \Phi_k(t) \dd k.
\end{equation}
This integral shows how to express $f(t)$ in terms of its
{\it Fourier Transform} $\hat{f}_k$. We should be clear on what this
integral means.  
It specifies a set of basis functions $\Phi_k(t)$ and an associated set of
coefficients $f_k$, such that the function $f(t)$ can be reconstructed
from the basis functions.  We can compute
the Fourier transform $f_k$ and forget the originial information $f(t)$,
being confident that $f(t)$ can be perfectly reconstructed from the
information on $f_k$.

But how can we compute the Fourier Transform $f_k$ associated
with a function $f(t)$?  Though
the expression is well-known, we'll briefly derive it here because it
illuminates some of the properties of Fourier transforms which will
generalize to KL tranforms.

To begin, we'll multiply both sides of Equation~\ref{eq:FT_1D} by the
basis function $\Phi^*_{k^\prime}(t)$, and integrate over all $t$.
Here $\Phi^\ast$ denotes the complex conjugate of $\Phi$.  This gives
\begin{equation}
  \int_{-\infty}^\infty \dd t \Phi^\ast_{k^\prime}(t) f(t)
  = \int_{-\infty}^\infty \dd t \Phi^\ast_{k^\prime}(t)
  \int_{-\infty}^\infty \dd k \hat{f}_k \Phi_k(t).
\end{equation}
Switching the order of integration and rearranging the right-hand-side
terms, we find
\begin{equation}
  \label{eq:IFT_deriv1}
  \int_{-\infty}^\infty \dd t \Phi^\ast_{k^\prime}(t) f(t)
  = \int_{-\infty}^\infty \dd k \hat{f}_k
  \int_{-\infty}^\infty \dd t \Phi^\ast_{k^\prime}(t)\Phi_k(t)
\end{equation}
Inserting the expression for $\Phi_k$ gives
\begin{eqnarray}
  \int_{-\infty}^\infty \dd t \Phi^\ast_{k^\prime}(t) f(t)
  &=& \int_{-\infty}^\infty \dd k \hat{f}_k
  \left[\frac{1}{2\pi} \int_{-\infty}^\infty
  \dd t e^{i t (k - k^\prime)}\right]\nonumber\\
  &=& \int_{-\infty}^\infty \dd k \hat{f}_k \delta(k - k^\prime)
\end{eqnarray}
where in the last line we have used the definition of the dirac delta
function,
\begin{equation}
  \delta(k) \equiv \frac{1}{2\pi} \int_{-\infty}^\infty e^{ikt} \dd t.
\end{equation}
Computing the trivial integral over the delta function, and relabeling
$k^\prime \to k$ yields the familiar result for the Fourier Transform:
\begin{equation}
  \label{eq:IFT_1D}
  f_k = \frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty f(t) e^{-ikt} \dd t.
\end{equation}

Equation~\ref{eq:IFT_1D} shows how to compute the Fourier transform
$f_k$ for a given $f(t)$.  But one might wonder if this is a unique
result.  Could there be many different valid Fourier transforms for a given
continuous function?

Let's assume that given a function $f(t)$, there are two valid Fourier
transforms, given by $f_k$ and $f^\prime_k$.  In this case, from
Equation~\ref{eq:FT_1D} we have
\begin{equation}
  f(t) - f(t) = \int_{-\infty}^\infty (f_k - f^\prime_k) \Phi_k(t) \dd k = 0
\end{equation}
Similarly to above, we can multiply by $\Phi^\ast_{k^\prime}(t)$,
integrate over all $t$, and extract a delta function to yield:
\begin{equation}
  \int_{-\infty}^\infty (f_k - f^\prime_k) \delta(k - k^\prime) \dd k = 0.
\end{equation}
Collapsing the integral we find that $f_k = f^\prime_k$ must hold for all $k$;
that is, the Fourier transform for continuously integrable functions
$f(t)$ is unique\footnote{The uniqueness property does not necessarily
hold for arbitrary functions $f(t)$ which are not piecewise continuous
or square-integrable.}.

Above, we have shown the case of continuous Fourier Transforms on an
unbounded domain $x \in (-\infty, \infty)$.  Very similar results can
be derived on bounded domains, i.e.~$x \in (a, b)$.  The primary difference
is that the infinite integral over continuous $k$ becomes a finite sum
over discrete $k$, and the basis functions are given by
\begin{equation}
  \Phi_k(x) = \exp\left[\frac{2\pi i k (x - a)}{b - a}\right]
\end{equation}
with a Fourier series expansion
\begin{equation}
  \label{eq:FS_1D}
  f_{(a, b)}(x) = \sum_{k=-\infty}^\infty f_k \Phi_k(x)
\end{equation}
and coefficients given by
\begin{equation}
  \label{eq:IFS_1D}
  f_k = \frac{1}{b - a}\int_a^b f_{(a, b)}(x) \Phi^\ast_k(x) \dd x
\end{equation}

